Tracy: A Business-driven Technical Debt Prioritization Framework

Technical debt is a pervasive problem in software development. Software development teams have to prioritize debt items and determine whether they should address debt or develop new features at any point in time. This paper presents "Tracy", a framework for the prioritization of technical debt using a business-driven approach built on top of business processes. The current stage of the proposed framework is at the beginning of the third phase of Design Science Research, which is usually divided into the phases of exploration, engineering, and evaluation. The exploration and engineering phases involved the participation of 49 professionals from 12 different groups of three companies. The initial evaluation shows that the presented framework is coherent in its structure and that its results contribute to business-driven decision making on technical debt prioritization.

==> body/body.tex <==
%\subsection{Annotation}


% During DSR's exploratory phase, we had the opportunity to understand several different business models, business processes, and metrics. The phase began with structured interviews and focus groups with one to three business participants. They were asked to enlist all products and services which they are responsible for. Besides that, they were asked to explain how these product and service create value for their customers and company. We discussed if business aspects must be taken into account when deciding about technical debt creation or payment. The objective of these discussions was to understand the perception of the value created by the systems and services. 

%During these first meetings, various participants made explicit that ``core'' functionalities must be taken into account and should not incur in risk \todo{CT: not sure what ``incur in risk'' means.}. Managers and participants with technical background tend to override the concepts of a business process and core functionalities. It is clear that the core functionalities are implementing important business processes. \todo{CT: Are these the ``findings'' from this work? I'm not sure what role this section plays in the overall paper... If they are findings, we need to say more about how exactly they were determined. But if the contribution is the framework, I'm not sure we need these?}

%Another main point in decision making is related to the ``customer profile'' and the trade-off between current metrics and potential metrics. For example, should I accept technical debt that degrades the performance of a system which will duplicate the scale in a few months? But we need to take it to create a pilot-project in short time to achieve a business opportunity. So, we must accept the performance debt, but it must be prioritized in the next few development cycles. 

%All groups agreed that it is necessary to make concrete their perception about the value of the systems and services and the value provided by them to the company and its customers. It became clear that in many situations, the participants had different perceptions about the business value of a system, a business priority, or the value of different customers. 

%It is necessary to use concrete metrics to decide and to communicate subjective evaluations behind decision making.

%Another highlight from these exploratory interventions was that the systems and services usually have a different business value from their business processes. For example, if we have an e-commerce system which supports the "sales" business process, it creates a positive business value like "revenue," but the system itself may be related to a business opportunity (e.g., the company may have strategic plans to reuse it to reach new markets). Or the system may have a "cost," an SLA regarding availability which may incur in penalties and loss. So, the business impact or the business value of a system is the union of the business value of the IT system or service and the value of the business processes supported by them.

%During the exploration phase, we identified dozens of different business processes and dozens of business metrics. Basically, since each business process creates business value, we may have at least one business metric for each process. And we can relate each metric with immediate, short, medium, and long-term decisions. So, it became obvious that the solution for prioritizing technical debt should be simple. It is not feasible to aggregate a big number of variables to make decisions (although this is what happens in subjective decisions).


